Continuous Linear Finite Element Method for Biharmonic Problems on Surfaces

This paper presents an innovative continuous linear finite element approach to effectively solve biharmonic problems on surfaces. The key idea behind this method lies in the strategic utilization of a surface gradient recovery operator to compute the second-order surface derivative of a piecewise continuous linear function defined on the approximate surface, as conventional notions of second-order derivatives are not directly applicable in this context. By incorporating appropriate stabilizations, we rigorously establish the stability of the proposed formulation. Despite the presence of geometric error, we provide optimal error estimates in both the energy norm and $L^2$ norm. Theoretical results are supported by numerical experiments.

==> teshared.tex <==
% Packages and macros go here
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathrsfs}
%\usepackage{epsfig}
\usepackage{enumitem}
%\usepackage{diagbox}
\usepackage{cases}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{stmaryrd}
\usepackage{xparse}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Linear FEM for biharmonic problem on surfaces}

\title{Continuous Linear Finite Element Method for Biharmonic Problems on Surfaces}
%
%\author{Ying Cai\thanks{Beijing Computational Science Research Center, Beijing 100193, China(\email{ycai@csrc.ac.cn}).}
%\and Hailong Guo\thanks{School of Mathematics and Statistics, The University of Melbourne, Parkville, VIC 3010, Australia(\email{hailong.guo@unimelb.edu.au}).}
%\and Zhimin Zhang\thanks{Beijing Computational Science Research Center, Beijing 100193, China(\email{zmzhang@csrc.ac.cn}) and  Department of Mathematics, Wayne State University, Detroit, MI 48202, USA(\email{ag7761@wayne.edu}).}
%}
